Differentiable Reasoning over a Virtual Knowledge Base

We consider the task of answering complex multi-hop questions using a corpus as a virtual knowledge base (KB). In particular, we describe a neural module, DrKIT, that traverses textual data like a KB, softly following paths of relations between mentions of entities in the corpus. At each step the module uses a combination of sparse-matrix TFIDF indices and a maximum inner product search (MIPS) on a special index of contextual representations of the mentions. This module is differentiable, so the full system can be trained end-to-end using gradient based methods, starting from natural language inputs. We also describe a pretraining scheme for the contextual representation encoder by generating hard negative examples using existing knowledge bases. We show that DrKIT improves accuracy by 9 points on 3-hop questions in the MetaQA dataset, cutting the gap between text-based and KB-based state-of-the-art by 70%. On HotpotQA, DrKIT leads to a 10% improvement over a BERT-based re-ranking approach to retrieving the relevant passages required to answer a question. DrKIT is also very efficient, processing 10-100x more queries per second than existing multi-hop systems.

==> scratch.tex <==
What are the main results:
- extension of PIQA to multi-hop case.
- runtime over existing multi-hop models.
- Wikimovies / WebQSP.

Methodological contributions:
- A PIQA system trained specifically to answer slot-filling
queries using distant supervision. (hard negative sampling)
- A differentiable operator for relation following over the
trained dense + sparse index.
- Very efficient sparse implementation of the above.

How to frame the paper:
- KBs are important -- they allow reasoning
- But they are incomplete, so people look at text based methods
- This is both slow, and ad-hoc for reasoning
- We extend PIQA work in two ways -- first by restricting
the index to slot-filling queries, we show it is possible to
improve its quality, get higher results
-- second we extend it to the multi-hop case, but introducing
a novel differentiable operator for relation-following.
- Experiments:
-- We show that our slot-filling system outperforms prior
reading comprehension based methods.
-- We show that end-to-end learning against the index is 
effective, outperforming PIQA, cascaded, and template approaches,
for both 1-hop and 2-hop.
-- We also show our method is efficient.
-- Then we show two applications of the virtual KB,
learning to answer multi-hop NL queries, and doing joint
entity linking + QA.

How to talk about methods?
- Multi-hop Neural Query Executor (or something similar)
- Problem Definition: Given a text corpus X we want to be able
to execute queries which involve following a path of relations
starting from a set of entities.
-- give examples.
- previous approaches either parse the query separately, and
execute it separately.
- or do an iterative retrieve + read process.
-- both these methods assume intermediate supervision.
*this description puts the reader in a comparison to these methods
frame of mind*

What is our task:
- Is it complex QA -- answer a complex question q against a
corpus X, by softly decomposing it into a sequence of relations?
- In this case what is the benefit over graph-based approaches?
- speed, interpretability, compositionality.
- Or is our task itself executing ``soft'' complex queries
against a text corpus.

How are we different from previous approaches?
- previous approaches to multi-hop QA do iterative retrieval + reading
- this is slow, and requires supervision on the inference chain
- how would these methods deal with very large sets?
- e.g. mayors-of(cities-in(USA)).

**We should really discuss this in the context of PIQA**

What is the connection between KB-QA and PIQA?
- Our problem is to execute KB queries against a text corpus,
for completeness.
- By definition this involves large corpora (open-domain QA)
and multi-hop QA.
- This poses an efficiency challenge, part of which was dealt
by PIQA by decomposing the indexing part and query execution part.
- However, such an approach cannot be used to answer multi-hop queries
because information in the index is local.
- One solution is to parse the query and execute the different parts
separately.
- But this way we cannot do end-to-end learning, and we need
intermediate supervision.

What is PIQA?
- An open-domain QA system which indexes the corpus separately
and queries separately, for efficiency at test time.
- Information in the index is, by definition, local since the
contexts of the phrases are local.
- This means they cannot be used to answer queries which involve
disparate pieces of information.
- give examples.

What we do?
- We extend PIQA to the multi-hop case.
- We also restrict the index to slot-filling queries.
- Results of a MIPS operation can be viewed as a weighted
set of entities.
- Doing multihop is iteratively constructing queries from a weighted
set of entities and a ``soft'' relation representation.

But why only slot-filling?
- That is our task.

What are our contributions?
- Results of a MIPS query can be viewed as a weighted set of mentions
- Using coreference we can aggregate to a weighted set of entities
- We can decompose the MIPS operation along weighted sets of entities
and a ``soft'' relation vector.
- Then mapping an input set of entities to an output set of related
entities becomes a sparse matrix vector multiplication.
- Decomposing the MIPS operation into entities and relations
also provides a natural way to construct hard negatives for training,
which shows empirical improvements over random sampling (and
PIQA negatives?).
- Also suggests a novel mechanism for generalizing to unseen relations
based on tail type seeds.

- No need for too many details in the intro
- We represent intermediate results of a complex query as a weighted
sets of entities.
- We decompose the score function for ranking answers in the index into
two components -- one using a query over the set of entities,
and the other over a ``soft'' representation of the relation.
- Then we further aggregate the results of the MIPS back into a weighted
set of entities using coreference.

